Prefill-Time Intervention for Mitigating Hallucination in Large Vision-Language Models

Large Vision-Language Models (LVLMs) have achieved remarkable progress in visual-textual understanding, yet their reliability is critically undermined by hallucinations, i.e., the generation of factually incorrect or inconsistent responses. While recent studies using steering vectors demonstrated promise in reducing hallucinations, a notable challenge remains: they inadvertently amplify the severity of residual hallucinations. We attribute this to their exclusive focus on the decoding stage, where errors accumulate autoregressively and progressively worsen subsequent hallucinatory outputs. To address this, we propose Prefill-Time Intervention (PTI), a novel steering paradigm that intervenes only once during the prefill stage, enhancing the initial Key-Value (KV) cache before error accumulation occurs. Specifically, PTI is modality-aware, deriving distinct directions for visual and textual representations. This intervention is decoupled to steer keys toward visually-grounded objects and values to filter background noise, correcting hallucination-prone representations at their source. Extensive experiments demonstrate PTI's significant performance in mitigating hallucinations and its generalizability across diverse decoding strategies, LVLMs, and benchmarks. Moreover, PTI is orthogonal to existing decoding-stage methods, enabling plug-and-play integration and further boosting performance. Code is available at: https://github.com/huaiyi66/PTI.

==> tables/analysis_Interp_imgValue.tex <==
\begin{figure}[h] % Use [htbp] for placement flexibility within the column
    \centering % Center everything within the figure environment


    \begin{minipage}[t]{\linewidth} % Slightly less than half width for spacing
        \centering
        % The height H/2 is implicitly handled by scaling width W
        % Assuming aspect ratio makes height proportional to width reduction
        \includegraphics[width=\linewidth]{imgs/mask_CHAIRi_llava.pdf} 
        % Optional: \vspace{-3pt}
        % Optional: \subcaption{Bottom Left} \label{fig:sub1} % Requires subcaption package
    \end{minipage}% <--- IMPORTANT: % prevents adding space/newline
   
  
    % --- Overall Caption and Label ---
    \caption{Your overall figure caption here, describing all three images.}
    \label{tables:analysis_Interp_imgValue} % Use a unique label for the whole figure
    % Optional: Add negative vspace to reduce space after caption, like \vspace{-5pt}
\end{figure}

==> tables/analysis_Interp_imgkey.tex <==


\begin{figure}[h] % Use [htbp] for placement flexibility within the column
    \centering % Center everything within the figure environment

    % --- Top Figure (Full Column Width) ---
    % Use minipage for consistency, though not strictly required for a single image
    % \begin{minipage}{\linewidth} % Takes the full width of the current column
    %     \centering
    %     \includegraphics[width=\linewidth]{imgs/llava_chair_image_attn.pdf} % W, H
    %     % Optional: Add negative vspace if needed, like \vspace{-3pt}
    % \end{minipage} 

    \begin{minipage}[t]{0.49\linewidth} % Slightly less than half width for spacing
        \centering
        % The height H/2 is implicitly handled by scaling width W
        % Assuming aspect ratio makes height proportional to width reduction
        \includegraphics[width=\linewidth]{imgs/chair_img_attn_llava.pdf} 
        % Optional: \vspace{-3pt}
        % Optional: \subcaption{Bottom Left} \label{fig:sub1} % Requires subcaption package
    \end{minipage}% <--- IMPORTANT: % prevents adding space/newline
    \hfill % Adds flexible horizontal space, pushing minipages apart
    \begin{minipage}[t]{0.49\linewidth} % Slightly less than half width
        \centering
        \includegraphics[width=\linewidth]{imgs/chair_img_attn_deepseek.pdf}
        % Optional: \vspace{-3pt}
        % Optional: \subcaption{Bottom Right} \label{fig:sub2} % Requires subcaption package
    \end{minipage}
    
    \vspace{5pt} % Add some vertical space between the top and bottom rows

    % --- Bottom Row (Two Figures Side-by-Side) ---
    \begin{minipage}[t]{0.49\linewidth} % Slightly less than half width for spacing
        \centering
        % The height H/2 is implicitly handled by scaling width W
        % Assuming aspect ratio makes height proportional to width reduction
        \includegraphics[width=\linewidth]{imgs/pope_object_attn_llava.pdf} 
        % Optional: \vspace{-3pt}
        % Optional: \subcaption{Bottom Left} \label{fig:sub1} % Requires subcaption package
    \end{minipage}% <--- IMPORTANT: % prevents adding space/newline
    \hfill % Adds flexible horizontal space, pushing minipages apart
    \begin{minipage}[t]{0.49\linewidth} % Slightly less than half width
        \centering
        \includegraphics[width=\linewidth]{imgs/pope_object_attn_deepseek.pdf}
        % Optional: \vspace{-3pt}
        % Optional: \subcaption{Bottom Right} \label{fig:sub2} % Requires subcaption package
    \end{minipage}

    % --- Overall Caption and Label ---
    \caption{Your overall figure caption here, describing all three images.}
    \label{tables:analysis_Interp_imgkey} % Use a unique label for the whole figure
    % Optional: Add negative vspace to reduce space after caption, like \vspace{-5pt}
\end{figure}

==> tables/analysis_combine_v2.tex <==
\begin{table}[!ht]
    \vspace{-5pt}
    \centering
    \caption{Cross-models and Comb-methods generalization study. Performance on POPE \textit{Adversarial} subset. ``$\mathcal{L} \Longleftrightarrow \mathcal{Q}$'': We restrict our cross-model generalization analysis to LLaVA-1.5 and Qwen-VL-Chat, as they share identical KV cache dimensions.}
      \vspace{-5pt}
    \label{tab:analysis_combine}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccccccc}
        \whline
        \multirow{2}{*}{Setting}   & \multirow{2}{*}{Method} 
        % \multirow{2}{*}{Generalization}   & \multirow{2}{*}{Method} 
        &\multicolumn{2}{c}{LLAVA.} &\multicolumn{2}{c}{Qwen.} &\multicolumn{2}{c}{DeepSeek.}\\

        \cmidrule(r){3-4} \cmidrule(r){5-6}  \cmidrule(r){7-8}  
        % ~ & &  $\text{POPE}(adv) \uparrow$ & MME  &  $\text{POPE}(adv) \uparrow$ & MME  &  $\text{POPE}(adv) \uparrow$ & MME  \\
         \hline
        % \multirow{2}{*}{Cross-models} 
        \multirow{2}{*}{\makecell{Cross\\LVLMs}} 
        

& \cellcolor{mygray}Vanilla  &  \cellcolor{mygray}$75.40$  & \cellcolor{mygray}$-$   &  \cellcolor{mygray}$80.26$  & \cellcolor{mygray}$-$  &  \cellcolor{mygray}$82.73$  & \cellcolor{mygray}$-$  \\


&  PTI ($\mathcal{L} \Longleftrightarrow \mathcal{Q}$) 
& $75.53$ &  \textcolor{mygreen}{$\uparrow 0.13$}  
& $81.47$ & \textcolor{mygreen}{$\uparrow 1.21$}  
& $-$ & $-$  \\

        % \cline{2-8}
        \hline
        
        % \multirow{4}{*}{Comb-methods} 
        \multirow{4}{*}{\makecell{Integrated\\Methods}} 

& \cellcolor{mygray}PAI  \cite{liu2024paying}
& \cellcolor{mygray}$76.93$ & \cellcolor{mygray}$-$
& \cellcolor{mygray}$81.63$ & \cellcolor{mygray}$-$
& \cellcolor{mygray}$84.03$ & \cellcolor{mygray}$-$ \\


& {PAI \textit{w/} PTI} 
& $78.76$ & \textcolor{mygreen}{$\uparrow 1.83$}  
& {${82.30}$} & \textcolor{mygreen}{$\uparrow 0.67$}  
& {${84.60}$} & \textcolor{mygreen}{$\uparrow 0.57$} \\

& \cellcolor{mygray}VISTA  \cite{li2025hidden}
& \cellcolor{mygray}$75.53$ & \cellcolor{mygray}{$-$} 
& \cellcolor{mygray}$80.80$ & \cellcolor{mygray}{$-$}
& \cellcolor{mygray}$84.80$ & \cellcolor{mygray}{$-$}  \\

& {VISTA \textit{w/} PTI} 
& $76.33$ & \textcolor{mygreen}{$\uparrow 0.80$}  
& $80.96$ & \textcolor{mygreen}{$\uparrow 0.16$} 
& {${85.56}$} & \textcolor{mygreen}{$\uparrow 0.76$}    \\


        \whline
        \end{tabular}
    }
    % \textsuperscript{*}{\ud{\raggedleft{\scriptsize{Note: ``LLAVA.'': LLAVA-1.5, ``Qwen.'': Qwen-VL-Chat, ``DeepSeek.'': DeepSeek-VL-Chat.}}}}
      \vspace{-10pt}
\end{table}
